Fact or Fiction? Can LLMs be Reliable Annotators for Political Truths?

Political misinformation poses significant challenges to democratic processes, shaping public opinion and trust in media. Manual fact-checking methods face issues of scalability and annotator bias, while machine learning models require large, costly labelled datasets. This study investigates the use of state-of-the-art large language models (LLMs) as reliable annotators for detecting political factuality in news articles. Using open-source LLMs, we create a politically diverse dataset, labelled for bias through LLM-generated annotations. These annotations are validated by human experts and further evaluated by LLM-based judges to assess the accuracy and reliability of the annotations. Our approach offers a scalable and robust alternative to traditional fact-checking, enhancing transparency and public trust in media.

==> hyper.tex <==
\begin{table}[h]
    \centering
    \caption{Hyperparameters  for annotators}
    \begin{tabular}{|l|l|}
        \hline
        \textbf{Hyperparameter} & \textbf{Typical Range/Options} \\
 &\\\hline
        \hline
        Model Names and Sizes& Llama3.1 8B , .. ..., FILL IN for others \\
        \hline
        Max Output Tokens & what was that? see code, i guess 500/? since categorical table few tokens an explaination take 200-400 tokens\\
        \hline
        Decoding Type & Greedy, Sampling ??? find \\
        \hline
        Top-k & 10-100 \\
        \hline
        Temperature & 0.0-2.0  [ plz fill it, lower the better]\\
 Batch processing&we did batch processing with asyncio [ref] to do labeling. it is done in batch of 10.\\
        \hline
        Stop Sequences & Custom (e.g. "\textbackslash n", ".", "END") \\
    \end{tabular}
    \label{tab:hyperparameters}
\end{table}
for LLM as judge, we used output token as -- , temperature 0.1 (to make it more determnistic), asked the LLM to give output in three runs to have more deterministic output, 

Judge params i used for gpt were below, write as line and remove image.
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Styles/image.png}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}

I see in your code , it is   max\_tokens=500,
